CDR-Bench: Evaluating Faithful Execution of Compositional, Order-Sensitive Data Refinement Recipes

Data refinement involves executing multi-step recipes over evolving text states, where both composition and execution order of processing operators determine the outcome. While existing benchmarks either isolate text editing or entangle it with code and tool execution, it remains unclear whether LLMs can directly and faithfully execute these compositional, order-sensitive data refinement recipes. To fill this gap, we introduce CDR-Bench, a comprehensive benchmark featuring 3,462 high-quality tasks spanning four real-world data refinement domains and 29 distinct operators. Our benchmark evaluates models across atomic, order-agnostic, and order-sensitive settings, leveraging deterministic reference outputs to enable exact evaluation. Experiments on 10+ state-of-the-art LLMs reveal consistent failure patterns: performance degrades sharply in compositional settings, and order-sensitive recipe success collapses. These findings underline that current LLMs lack the procedural faithfulness required for reliable compositional data refinement.

==> tables/real_scenario_main.tex <==
% \begin{table}[t]
% \centering
% \resizebox{0.95\columnwidth}{!}{
% \begin{tabular}{@{}l cc cc@{}}
% \toprule
% & \multicolumn{2}{c}{\textbf{PII Redaction}} & \multicolumn{2}{c}{\textbf{Hallucination}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% \textbf{Model} & Atomic & Comp & Atomic & Comp \\
% \midrule
% Claude Opus 4.5   & \underline{66.9} & \textbf{45.0} & 19.1 & \underline{22.2} \\
% Claude Opus 4.6   & 66.7 & \underline{44.4} & 16.7 & 20.0 \\
% Qwen3.6-Max       & \textbf{67.4} & 43.0 & \textbf{21.7} & 21.4 \\
% GPT-5.4           & 57.5 & 33.2 & 15.5 & 15.0 \\
% DeepSeek-V4-Flash & 55.6 & 38.0 & \underline{21.1} & 20.0 \\
% Kimi-K2.6         & 58.8 & 28.0 & 19.7 & \textbf{31.1} \\
% GLM-5             & 66.0 & 41.0 & 15.3 & 14.3 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Real-scenario evaluation (RS \%). Atomic: mean across atomic subtasks; Comp: compositional.}
% \label{tab:semantic_compact}
% \vspace{-0.5\baselineskip}
% \end{table}

\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.08}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l cc cc cc cc@{}}
\toprule
\textbf{Model}
& \multicolumn{2}{c}{\textbf{PII}}
& \multicolumn{2}{c}{\textbf{Hallu.}}
& \multicolumn{2}{c}{\textbf{Safety}}
& \multicolumn{2}{c}{\textbf{Rubric}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
& At. & Cp.
& At. & Cp.
& At. & Cp.
& At. & Cp. \\
\midrule

\rowcolor{closedBg}
\multicolumn{9}{@{}c@{}}{\textit{Closed-Source Models}} \\
\addlinespace[1pt]

Claude Opus-4.7
& 74.5 & 50.6
& 26.1 & 24.7
& 77.0 & 48.0
& 51.3 & 7.7 \\

Claude Sonnet-4.6
& 69.7 & 47.2
& 25.7 & 24.7
& 75.0 & 46.0
& 42.7 & 2.7 \\

Qwen3.6-Max
& 77.3 & 51.0
& 33.5 & 27.7
& 77.3 & 45.0
& 61.5 & 6.3 \\

GPT-5.5
& 69.6 & 51.8
& 24.6 & 21.0
& 72.0 & 46.0
& 50.2 & 5.7 \\

\midrule
\addlinespace[2pt]
\rowcolor{openBg}
\multicolumn{9}{@{}c@{}}{\textit{Open-Source Models}} \\
\addlinespace[1pt]

DeepSeek-V4-Flash
& 67.6 & 39.4
& 41.8 & 36.3
& 76.1 & 49.0
& 64.7 & 4.0 \\

Kimi-K2.6
& 69.2 & 34.2
& 31.2 & 23.3
& 74.2 & 49.3
& 51.9 & 1.3 \\

GLM-5
& 73.4 & 39.0
& 37.1 & 29.0
& 75.6 & 50.3
& 48.7 & 2.3 \\

Gemma-4
& 74.0 & 45.8
& 34.2 & 29.3
& 72.4 & 44.7
& 55.3 & 5.3 \\

Qwen3.6-27B
& 62.3 & 40.2
& 37.7 & 35.0
& 79.3 & 52.7
& 62.4 & 3.7 \\

Qwen3.6-35B-A3B
& 60.9 & 25.0
& 35.9 & 37.0
& 76.8 & 48.3
& 63.1 & 2.0 \\

\bottomrule
\end{tabular}
}

\caption{Real-World scenario evaluation results (RS@3 \%) across four domains: PII Redaction (PII), Hallucination Processing (Hallu.), Safety Tagging (Safety), and Rubric Scoring (Rubric). For each domain, At.\ denotes the atomic-subtask average and Cp.\ denotes the compositional task. Models are grouped into closed-source and open-source systems. The atomic-to-compositional gaps are visualized in Figure~\ref{fig:semantic_atomic_comp_drop_by_domain}.}
\label{tab:semantic_compact}
\vspace{-0.5\baselineskip}
\end{table}
